iFacetSum: Coreference-based Interactive Faceted Summarization for Multi-Document Exploration

We introduce iFacetSum, a web application for exploring topical document sets. iFacetSum integrates interactive summarization together with faceted search, by providing a novel faceted navigation scheme that yields abstractive summaries for the user's selections. This approach offers both a comprehensive overview as well as concise details regarding subtopics of choice. Fine-grained facets are automatically produced based on cross-document coreference pipelines, rendering generic concepts, entities and statements surfacing in the source texts. We analyze the effectiveness of our application through small-scale user studies, which suggest the usefulness of our approach.

==> figures/consent_form.tex <==
Dear participant

You are being invited to participate in a research study titled" CorExplorer 1". This study is being done by  Eran H., Ori S., and Hadar R. from the University of Bar-Ilan.
 
This study consists of 4 parts. You will recieve explanation ob each part. 

The study will take you approximately 30 minutes to complete.
 
To the best of our ability your answers in this study will remain confidential.  We don't collect any personal information. Your participation in this study is completely voluntary and you can withdraw at any time. 
If you have questions about this project you may contact the researcher(s),Hadarg@gmail.com.  
 
By clicking “I agree” below you are indicating that you are at least 18 years old, have read and understood this consent form and agree to participate in this research study. 
You may print a copy of this page for your records.
 
We thank you for your time. 

==> figures/figPopovers.tex <==
\begin{figure*}[t!]
    \centering
    \resizebox{\linewidth}{!}{
        \begin{subfigure}[]{\columnwidth}
            \centering
            \includegraphics[width=(\columnwidth)]{figures/original_sentences.png}
        \end{subfigure}\hfill
        \begin{subfigure}[]{\columnwidth}
            \centering
            \includegraphics[width=(\columnwidth)]{figures/original_document.png}
        \end{subfigure}\hfill
        \begin{subfigure}[]{\columnwidth}
            \centering
            \includegraphics[width=(\columnwidth)]{figures/history.png}
        \end{subfigure}\hfill
    }
    \caption{There are three pop ups that can be opened from the summary component. The left screenshot shows the original sentences feature, which describes which sentences were used to create the summary. The middle screenshot shows the original document feature, which enables the user to get more context by reading the full document, while the sentences that were used to create the summary are marked in red. The right shows the history feature, which enables the user to easily collect the information they discovered over time.}
    \label{fig_summary_popups}
\end{figure*}


==> figures/tabSUSQuestionnaire.tex <==
\begin{table*}[]

\begin{tabularx}{\linewidth}
{
 | > {}l 
 | > {}X |
}
\hline
\textbf{\#} & \textbf{SUS Question}                                                                  \\ \hline
1  & I think that I would like to use this system frequently.                      \\ \hline
2  & I found the system unnecessarily complex.                                     \\ \hline
3  & I thought the system was easy to use.                                         \\ \hline
4  & I think that I would need the support of a technical person to be able to use this system. \\ \hline
5  & I found the various functions in this system were well integrated.            \\ \hline
6  & I thought there was too much inconsistency in this system.                    \\ \hline
7  & I would imagine that most people would learn to use this system very quickly. \\ \hline
8  & I found the system very cumbersome to use.                                    \\ \hline
9  & I felt very confident using the system.                                       \\ \hline
10 & I needed to learn a lot of things before I could get going with this system.  \\ \hline
\end{tabularx}
\caption{Standard SUS questionnaire \cite{brooke1995sus}.}
\label{table_sus_questionnaire}
\end{table*}


==> figures/tabSummarizationQualityQuestions.tex <==
\begin{table}[h!]
\begin{tabularx}{\columnwidth}
{|c|l|X|}
\hline
\textbf{\#} & \textbf{Aspect} & \textbf{Task Question} \\ \hline
1  & Grammatically           & The summary should have no datelines, system-internal formatting, capitalization errors or obviously ungrammatical sentences (e.g., fragments, missing components) that make the text difficult to read. \\ \hline
2  & Non-redundancy          & There should be no unnecessary repetition in the summary. Unnecessary repetition might take the form of whole sentences that are repeated, or repeated facts, or the repeated use of a noun or noun phrase (e.g., “Bill Clinton”) when a pronoun (“he”) would suffice. \\ \hline
3  & \makecell[tl]{Referential\\clarity}     & It should be easy to identify who or what the pronouns and noun phrases in the summary are referring to. If a person or other entity is mentioned, it should be clear what their role in the story is. So, a reference would be unclear if an entity is referenced but its identity or relation to the story remains unclear. \\ \hline
4  & Focus                    & The summary should have a focus; sentences should only contain information that is related to the rest of the summary.    \\ \hline
5  & \makecell[tl]{Structure and\\Coherence} & The summary should be well-structured and well-organized. The summary should not just be a heap of related information, but should build from sentence to sentence to a coherent body of information about a topic.        \\ \hline
6  & Factuality              & The sentence should stay true to the source text ; information provided in the sentence should have evidence in the source text, even if phrased differently.          \\ \hline
\end{tabularx}
\caption{Summaries quality questionnaire, first 5 aspects are based on \cite{dang2006DUCoverview}. }
\label{table_summarization_quality_questionnaire}
\end{table}


==> figures/tabTimingQuestionnaire.tex <==
\begin{table}[ht]
\begin{tabularx}{\columnwidth}
{|c|X|c|}
\hline
\textbf{\#} & \textbf{Task Question} & \textbf{Score} \\ \hline
1 & Which system was \textit{easier to use} in order to get the desired result?               & 5.5  (1.73)    \\ \hline
2 & With which system was it easier for you to get an \textit{overview of the topic}?         & 5.0    (2.30) \\ \hline
3 & With which system was it easier for you to get \textit{detailed information} about a subtopic of interest? & 5.25 (0.9) \\ \hline
4 & If you had to learn about or explore a new topic, \textit{which system would you choose}? & 5.25 (0.95) \\ \hline
\end{tabularx}
\caption{System comparison experiment questionnaire, with the average and (StD) results. The scale ranges from 1 to 7 where 1 means DocFetcher is preferred and 7 means \App{} is preferred. }
\label{table_timing_questions}
\end{table}


==> figures/tabUsefulnessQuestionnaire.tex <==
\begin{table}[]
\begin{tabularx}{\columnwidth}
{
 | > {}l 
 | > {}X |
}
\hline
\textbf{\#} & \textbf{Task Question}                                                                                                            \\ \hline
   & For the requirements of the given task, how useful was each of the following components between 1 (not useful at all) and 5 (very useful). \\ \hline
1  & Facets.                                                                                                                                    \\ \hline
   & Overall, the summaries output by the system were: between 1 (I disagree) and 5 (I agree)                                                   \\ \hline
2  & Coherent.                                                                                                                                  \\ \hline
3  & Informative.                                                                                                                               \\ \hline
4  & Non-Redundant.                                                                                                                             \\ \hline
5  & Length is about right.                                                                                                                     \\ \hline
\end{tabularx}
\caption{Usefulness questions the users answered after each topic. }
\label{table_usefulness_questionnaire}
\end{table}
